A continuous integration and web framework in support of the ATLAS Publication Process

The ATLAS collaboration defines methods, establishes procedures, and organises advisory groups to manage the publication processes of scientific papers, conference papers, and public notes. All stages are managed through web systems, computing programs, and tools that are designed and developed by the collaboration. A framework called FENCE is integrated into the CERN GitLab software repository, to automatically configure workspaces where each analysis can be documented by the analysis team and managed by the relevant coordinators. Continuous integration is used to guide the writers in applying consistent and correct formatting when preparing papers to be submitted to scientific journals. Additional software assures the correctness of other aspects of each paper, such as the lists of collaboration authors, funding agencies, and foundations. The framework and the workflow therein provide automatic and easy support to the researchers and facilitates each phase of the publication process, allowing authors to focus on the article contents. The framework and its integration with the most up to date and efficient tools has consequently provided a more professional and efficient automatized work environment to the whole collaboration.

==> ANA-GENR-2018-01-PAPER-auxmat.tex <==
\part*{Auxiliary material}
\addcontentsline{toc}{part}{Auxiliary material}
%-------------------------------------------------------------------------------

In an ATLAS paper, auxiliary plots and tables that are supposed to be made public 
should be collected in an appendix that has the title \enquote{Auxiliary material}.
This information will appear on the public webpage, but will not be included
in the document submitted to arXiv and to the journal.


==> ANA-GENR-2018-01-PAPER-hepdata.tex <==
\section{HepData material}
%-------------------------------------------------------------------------------

This file is available for detailed tables etc.\ that are going to be
submitted to HepData or other similar destinations.

==> ANA-GENR-2018-01-PAPER-metadata.tex <==
% Turn off some chktex warnings.
% chktex-file 1 chktex-file 8 chktex-file 46
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used for an ATLAS note.
%-------------------------------------------------------------------------------

% Title
\AtlasTitle{A continuous integration and web framework in support of the ATLAS Publication Process}

% Draft version:
% Should be 1.0 for the first circulation, and 2.0 for the second circulation.
% If given, adds draft version on front page, a 'DRAFT' box on top of each other page, 
% and line numbers.
% Comment or remove in final version.
%\AtlasVersion{0.1}
%\linenumbers
% Abstract - % directly after { is important for correct indentation
\AtlasAbstract{%
  The ATLAS collaboration defines methods, establishes procedures, and organises advisory groups to manage the publication processes of scientific papers, conference papers, and public notes.
  All stages are managed through web systems, computing programs, and tools that are designed and developed by the collaboration.
  A framework called FENCE is integrated into the CERN GitLab software repository, to automatically configure workspaces where each analysis can be documented by the analysis team and managed by the relevant coordinators.  
  Continuous integration is used to guide the writers in applying consistent and correct formatting
  when preparing papers to be submitted to scientific journals.
  Additional software assures the correctness of other aspects of each paper, such as the lists of collaboration authors, funding agencies, and foundations. 
  The framework and the workflow therein provide automatic and easy support to the researchers and facilitates each phase of the publication process, allowing authors to focus on the article contents. The framework and its integration with the most up to date and efficient tools has consequently provided a more professional and efficient automatized work environment to the whole collaboration.
}

% Author - this does not work with revtex (add it after \begin{document})
% \author{The ATLAS Collaboration}

% Authors and list of contributors to the analysis
% \AtlasAuthorContributor also adds the name to the author list
% Include package latex/atlascontribute to use this
% Use authblk package if there are multiple authors, which is included by latex/atlascontribute
% \usepackage{authblk}
% Use the following 3 lines to have all institutes on one line
% \makeatletter
% \renewcommand\AB@affilsepx{, \protect\Affilfont}
% \makeatother
% \renewcommand\Authands{, } % avoid ``. and'' for last author
% \renewcommand\Affilfont{\itshape\small} % affiliation formatting

%Authors - OrcID

%1%
\author[f]{\AtlasOrcid[0000-0003-2927-9378]{Juan Pedro Araque Espinosa}}
%2%
\author[a]{Gabriel Baldi Levcovitz}
%3%
\author[i]{\AtlasOrcid[0000-0001-7345-7798]{Riccardo-Maria Bianchi}}
%4%
\author[d]{\AtlasOrcid[0000-0003-0903-8948]{Ian Brock}}
%5%
\author[b]{\AtlasOrcid[0000-0003-4058-5376]{Tancredi Carli}}
%6%
\author[f,g]{\AtlasOrcid[0000-0001-8491-4376]{Nuno Filipe Castro}}
%7%
\author[h]{\AtlasOrcid[0000-0002-3081-4879]{Alessandra Ciocio}}
%8%
\author[e]{Maurizio Colautti}
%9%
\author[a]{Ana Carolina Da Silva Menezes}
%10%
\author[a]{Gabriel De Oliveira da Fonseca}
%11%
\author[e]{Leandro Domingues Macedo Alves}
%12%
\author[b]{\AtlasOrcid[0000-0002-6596-9395]{Andreas Hoecker}}
%13%
\author[a]{Bruno Lange Ramos}
%14%
\author[a,f]{Gabriela Lemos L\'ucidi Pinh{\~a}o}
%15%
\author[a]{\AtlasOrcid[0000-0002-3511-0133]{Carmen Maidantchik}}

%16%
% \author[c]{\AtlasOrcid[0000-0002-0948-5775]{Fairouz Malek}\thanks{Contact editor: fmalek@lpsc.in2p3.fr}}
\author[c]{\AtlasOrcid[0000-0002-0948-5775]{Fairouz Malek}}
%17%
\author[j]{\AtlasOrcid[0000-0001-9211-7019]{Robert McPherson}}
%18%
\author[e]{Gianluca Picco}
%19%
\author[a]{Marcelo Teixeira Dos Santos}

%Affiliations
%RIO%
\affiliation[a]{Universidade Federal do Rio De Janeiro COPPE/EE/IF, Rio de Janeiro, Brazil}
%CERN%
\affiliation[b]{CERN}
%Grenoble%
\affiliation[c]{LPSC, Universit\'e Grenoble Alpes, CNRS/IN2P3, Grenoble, France}
%Bonn%
\affiliation[d]{Physikalisches Institut, Universit\"{a}t Bonn, Bonn, Germany}
%Udine%
\affiliation[e]{Dipartimento Politecnico di Ingegneria e Architettura, Universit\`a di Udine, Udine, Italy}
%LIP%
\affiliation[f]{Laborat\'orio de Instrumenta\c{c}\~ao e F\'isica Experimental de Part\'iculas, Lisbon, Portugal}
\affiliation[g]{Departamento de F\'isica, Escola de Ci\^encias, Universidade do Minho, Braga, Portugal}
%Berkely%
\affiliation[h]{Lawrence Berkeley National Laboratory and University of California, Berkeley, USA}
%Pittsburg%
\affiliation[i]{Department of Physics and Astronomy, University of Pittsburgh, Pittsburgh PA, USA.}
%Victoria%
\affiliation[j]{Department of Physics and Astronomy, University of Victoria, Victoria BC, Canada}

% JINST email
\emailAdd{fmalek@lpsc.in2p3.fr}

% ATLAS reference code, to help ATLAS members to locate the paper
\AtlasRefCode{GENR-2018-01}

% ATLAS note number. Can be an COM, INT, PUB or CONF note
\AtlasCoverSupportingNote{PO Glance Gitlab}{https://cds.cern.ch/record/2676784}

\PreprintIdNumber{CERN-OPEN-2020-007}

\PreprintIdNumber{2005.06989}


==> ChangeLog <==
2019-09-13  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 07-05-01.
	* Remove usage of tocloft package, as it can conflict with KOMA-Script.
	* Set default table of contents depth to section and add tocdepth option.
	* July update of publications (except CMS).
	* Fix up a number of references in ATLAS-useful.bib and add a few new ones.
	* Add some, but not all, of the ATLAS TDRs to ATLAS.bib.
	* Small updates to SUSY templates.
2019-05-21  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 07-04-00.
	* Tweak the logic of the backref option.
	Now off by default, except for draft documents.
2019-05-09  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 07-03-00.
	* April update of publications.
	* Tweak atlaslatex_update.sh to not overwrite help text with BASENAME.
	* A few fixes to references and detector description.
2019-03-19  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 07-02-00.
	* February update of publications.
	* Run 2 detector description added.
	* Update ATLAS-SUSY.bib and ATLAS-useful.bib.
2019-02-28  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 07-01-01.
	* Update ATLAS-SUSY.bib with correct Errata format and other fixes.
2019-02-22  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 07-01-00.
	* January update of publications.
	* Add option backref to atlasbiblatex.
	* Add commented out authorlist to paper template.
	* Add INT note templates for SUSY group. These are a WIP and subject to further change.
2019-01-11  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 07-00-00.
	* November update of publications.
	* Rewrite macros for creating cover and title pages.
	Copyright notice should now always be correctly positioned.
	Less space used for title etc.
	Tweaking of offsets should no longer be necessary.
	Warnings about overfull hboxes fixed.
	Previous version available as atlasdoc2.cls and atlascover2.sty.
	* Add \JHEP as a journal.
	* Always use paper=letter option for US paper size.
	* Some tweaks so turning on language editor comments should not change text width.

2018-11-30  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 06-00-00.
	* October update of publications.
	* Number and unit spacing in bib files changed to ~ instead of \;.
	* Use \text instead of \mbox, \textrm, \mathrm in bib files.
	* Use \(...\) instead of $...$ in template and bib files.
	* Use firstinits instead of giveninits as biblatex option for TeX Live < 2016 instead of 2015.
	* Moved atlaslatex_update.sh script to scripts subdirectory.
	* Added a script tex_dollars.py to convert $...$ to \(...\).

2018-10-29  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 05-09-00.
	* September update of publications.
	* Add INT note templates for EXOT group. These are a WIP and subject to further change.
	* Updated acknowledgements.
2018-10-11  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 05-08-00.
	* July and August updates of publications.
	* A few tweaks to box sizes to get the copyright more often in the right place.
	* BASENAME should be set correctly if Makefile is overwritten via atlaslatex_update.sh.
	* Added bib files ATLAS-useful.bib and ATLAS-SUSY.bib.
	* Start adding text snippets to new atlassnippets.sty style file.
	* Use latexmk to make documentation.
	* Changed instructions for references for big collaborations (only collaboration name).
	* Add microtype package to standard packages that are included.
	* Moved atlas_paper to atlaslatex-admin, as the ATLAS Style Guide should contain everything.
2018-08-02  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 05-07-00.
	* May and June updates of publications.
2018-05-15  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 05-06-00.
	* April updates of publications.
	* Start adding copyright statements and LICENSE so code can be made public.
	* atlas_physics has a UK and a US version.
	* Make \dif language sensitive.
2018-05-04  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 05-05-00.
	* March updates of publications.
	* Moved all old/obsolete style files to an obsolete directory.
	* Move bst directory with traditional BibTeX style files to obsolete.
	* Added \NIMA as a journal.
2018-03-16  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 05-04-00.
	* February updates of publications.
	* Add bookmarks to PDF file via hyperref.
	* Add a script atlaslatex_update.sh to be able to update your atlaslatex version.
	* Move old logos to an obsolete directory.
	* Move obsolete style files to same directory.
	* Move lineno.sty and authblk.sty to same directory.
2018-02-20  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 05-03-00.
	* January updates of publications.
	* Updated acknowledgements.
	* Fix language editor comments so that they also work in captions etc.
	* Tables document has captions above table.
2018-01-11  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 05-02-02.
	* December updates of publications.
	* Allow both cernpreprint and PAPER options.
	* Adjust some definitions to follow ATLAS Style Guide.
	* Added \tauhad, \taulep, \tauhadvis and \taup definitions.
	* Added \xspace to journal names in atlasjournal.sty.
	* Move \pileup to atlasmisc.sty.
	* \KT from atlasmisc.sty now \kperp.
	* \RcaloM now \Rcalom
2017-12-12  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 05-01-03.
	* CERN preprint ID corrected.
2017-11-30  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 05-01-02.
	* November update of publications.
	* Abstract in BOOK now properly justified.
	* Add atlascomment package for language editors.
	* Add option LANGEDIT (and LANGSHOW) to atlasdoc to turn on display of comments.
	* The atlasmetadefs.sty style file should no longer be necessary when using atlasdoc.
	* Moved atlasdoc1.cls and atlascover1.sty to obsolete directory.
2017-11-07  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 05-00-01.
	* September and October updates of publications.
	* Add a proper title page for the BOOK option.
	* Book abstract is put on a separate page.
	* Add atlasdraft option to indicate if the document is a draft.
	* Add option abstract, which should be set to false for books without an abstract.
	* A skeleton Auxiliary Material file is included by default for papers.
	* The auxmat option has been renamed to HEPDATA to reflect its usage.
	* Add percentspace option to atlaspackage so space between number and percent can be turned off.
	* Add \MADGRAPHV and \MGMCatNLOV to atlasmisc.sty.
	* Move from scrpage2 to scrlayer-scrpage package for TeX Live > 2014.
	* Titles for report and misc bibliography entries by default in italics.
	* Pages abbreviation removed also for "english" as language.

2017-09-29  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 04-02-00.
	* August 2017 update of publications.
2017-08-23  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 04-01-00.
	* July 2017 update of publications.
	* Add command to make sure \ell is shown using PDF figures.
2017-07-21  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 04-00-00.
	* Switch from bibtex to biber as the standard biblatex backend.
	* Move bibtex/bib to bib and bibtex/bst to bib/bst.
	* Add Errata to ATLAS.bib. This only works properly with biblatex.
	* Reorganise Makefile to use separate metadata files for notes and paper.
	* Add ability to use latexmk in Makefile.
	* Separate templates for paper draft and notes.
	* Use same document template for texmf version.
	* Add defaultsups option to newtxtext so multiple authors work properly with TeX Live 2017.
	* Add more version variants to MC generator macros.
	* Changes to atlasmetadefs,sty so that it works when coverpage is turned off.
	* Change group-minimum-digits option for siunitx from 4 to 5.
	* Add some explanation on use of group-minimum-digits to tables documentation.
	* Start adding some documentation about useful packages to ATLAS LaTeX documentation.

2017-07-03  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 03-03-00.
	* June 2017 update of publications.
2017-05-30  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 03-02-00.
	* May 2017 update of publications.
2017-05-16  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 03-01-00.
	* Small update to detector description.
	* Include ATLAS bibliography files by default.
	* April 2017 update of publications.
2017-03-31  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 03-00-01.
	* atlaslatex is now maintained in Git.
	* February and March 2017 update of publications.
2017-02-16  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 03-00-00.
	* Default TeX Live version changed to 2016 to match arXiv.
	* October 2016 to January 2017 updates of ATLAS publications.
	* eVkern option selected by default when using txfonts.
	* Some options to add more real estate for the abstract on the title page.
	* Add option datetop to put the date at the top of the title page.
	* Add option titlepage to select normal or smaller fonts for the title page.
	* Fix problem when using subcaption with list of figures or tables.
	* Move maxbibnames and block options to atlasbiblatex.sty.
	* Set maxbibnames=5 by default to conform with current recommendations.
	* Added option subfig to atlaspackage, so all subfigure packages can be turned off.
	* More generic font commands on cover and title pages.
	* Add option to reduce font sizes on title page.
	* Add option to include mhchem early for TeX Live 2014.
	* Add some more temporary files that come from latexmk and TextMate to the list to clean up.
	* Small change to atlasdoc1.cls to get date printed when KOMA-Script is not used.

2016-10-10  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 02-00-01.
	* Fixes known bugs in version 02-00-00. Tested on usual platforms.
	* Add atlascover1.sty to go with atlasdoc1.cls.
	* September update of publications.
2016-09-21  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 02-00-00.
	* Drop standard LaTeX classes - only use KOMA-Script.
	* atlasdoc1 can use LaTeX classes, but does not support BOOK.
	* Add BOOK option for book as base class for things like LOIs and TDRs.
	* Use the command "make newbook" to create such a document.
	* This release is not perfect. You have to steer the coverpage from class options.
	Hopefully this will be fixed in the next release.

2016-09-07  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 01-08-02.
	* June, July, August updates of ATLAS and CMS publications.
2016-08-23  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 01-08-01.
	* New style file atlasjetetmiss.sty with definitions from the Jet/ETmiss group.
	* A number of definitions from the Jet/ETmiss group were added to atlasmisc.sty,
	atlasparticle,sty and atlasprocess.sty.
	* Add option eVkern to atlaspackage to move 'e' and 'V' closer
	together in eV and its variants, e.g. GeV.
	* Add options hepparticle and hepprocess to atlasphysics,
	which use particle names from the hepparticle package.
	* Update definitions of \GeV etc. in atlasunit.sty (even though you
	shouldn't be using them - use siunitx instead)!
	* Add some discussion about \it, \rm, \tt etc. errors in TeX Live 2016.
2016-06-15  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 01-07-13.
	* Add location and address options to atlasbiblatex.
	* Do not print month in references (when using biblatex).
	* Correct volume number for JHEP (without year).
	* May updates of ATLAS and CMS publications.
2016-05-20  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 01-07-12.
	* Add maxbibnames option to atlaspackage.
	* April updates of ATLAS and CMS publications.
2016-05-09  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 01-07-11.
	* Switch to new ATLAS logo.
	* March updates of ATLAS and CMS publications.
2016-03-22  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 01-07-10.
	* February updates of ATLAS and CMS publications.
	* Small fix to link from journal information to DOI.
	* Small updates to documentaton on ATLAS LaTeX.
	* Add xspace to aMC@NLO.
	* Adjusted journal examples and documentation to use	\ATLASLATEXPATH.
	This makes compilation with Windows easier, as links are no longer needed.
2016-01-29  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 01-07-09.
	* December and January updates of ATLAS and CMS publications.
2015-12-19  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 01-07-08.
	* October and November updates of ATLAS and CMS publications.
	* Suppress issue number in journal volume.
	* Add a couple more Herwig symbols.
2015-11-21  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 01-07-07.
	* August and September updates of ATLAS and CMS publications.
	* Updated acknowledgements.
	* Some help for JINST publications added.
	* Change to CC-BY-4.0.
	* Add commented out code to get institutes on one line for title page.
2015-07-31  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 01-07-06.
	* June and July updates of ATLAS and CMS publications.
	* Improve siunitx option setting for TeX Live 2011 (arXiv version).
	* A few fixes so that things (sort of) work with TeX Live earlier than 2009.
	* Move \pdfoutput=1 command even earlier in template.
	* Small tweak of title page header for long note numbers.
	* Add \App etc. to atlasxref.sty for appendices.
	* Add some more Monte Carlos to atlasmisc.sty.
	* Add some more units to atlas_physics for testing.
	* Add some documentation about JINST.
	* Adjust things so documentation compiles for TeX Live versions.
	* Tweaks for subtables, so that labels are correct.
2015-06-22  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 01-07-05.
	* Monthly update of ATLAS and CMS publications.
	* Only print first page in biblatex bibliography.
	* Add (unfortunately) support for TeX Live 2007 and earlier -needed by JINST.
	* Add a few more MC generators to atlasmisc.sty.
	* Add macros for cross-referencing appendices to atlasxref.sty.
2015-06-10  Ian Brock  <Ian.Brock@cern.ch>
	* Set subfig and subcaption options so that \ref and \subref work as in subfigure.
	* Add a bit more documentation on subfigures.
2015-06-03  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 01-07-04.
	* Monthly update of ATLAS and CMS publications.
	* Biblatex option only works as of 2014 and not 2013.
	* Add comment to documentation about APS journals.
	* Add \ppbar as symbol.
2015-04-29  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 01-07-03.
	* Monthly update of ATLAS and CMS publications.
	* Do not use tabular on cover page for supporting notes.
	* A few minor improvements to template comments.
	* Improve steering of what is done if latex command is used in Makefile.
	* Check if biblatex is loaded in atlasbiblatex.
2015-03-20  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 01-07-02.
	* A few small fixes to the bib files.
	* Move from atlas-paper.bib to ATLAS.bib everywhere.
	* Document better how to switch between subfigure, subfig and subcaption.
	* Move acknowledgements archive to the admin tree
2015-03-17  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 01-07-01.
	* Line numbers turned off by mistake in version 01-07-00.
	* Added preliminary version of ATLAS.bib.
	* Add block option to atlaspackage.
2015-03-13  Ian Brock  <Ian.Brock@cern.ch>
	* Updated PUB and CONF note bib files. ATLASbib comes a bit later.
	* Improve instructions for arXiv and CERN preprint.
2015-03-09  Ian Brock  <Ian.Brock@cern.ch>
	* Tag as version 01-07-00.
	* ATLAS CONF and PUB notes bib files included. Journal	publications to come.
	* maketitle=false is now the default option to avoid problems with
	siunitx and units in the title/abstract.
	* Added a few instructions on CERN preprint preparation.
	* Add option detect-all to siunitx.
	* Improve cross-referencing macros a bit.
	* Some adjustments and additions made to the standard Makefile
	* Added a new command "make cleanepstopdf" to delete PDF files
	made automatically from EPS files.
2015-03-02 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 01-06-03.
	* Allow BSM and bsm as options for atlasphysics.sty.
2015-02-23 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 01-06-02.
	* Add a variable \ATLASLATEXPATH which contains the directory for style files.
	This can be used instead of the texmf option and is more flexible.
	* Print note after URL and eprint.
	* Add biblatex option to turn off eprint.
	* Add some documentation on different directory options.
2015-02-08 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 01-06-01.
	* Remove contact editor from cover page.
	* Adjust things so that only TeX Live version has to be specified.
	* Remove 'make new2009' target. Use 'make new TEXLIVE=2009' etc instead.
	* Remove atlas-document-2009.tex, as texlive=YYYY now steers everything.
	* Should work back to TeX Live 2009. Before that have to turn off biblatex.
2015-02-01 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 01-06-00.
	* Several tweaks to the cover page so that it can cope better with a long abstract.
	* Add option coverfontsize to steer the base font size for the cover pages.
	* Add PAPER and NOTE as options to atlasdoc, so that ATLAS Paper gets printed on title page.
	* Adjust options for placement and number of floats on a page.
	* Only print journal name for paper drafts.
	* Add package ifthen as a required package.
2014-12-23 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 01-05-03.
	* Add acknowledgements.
2014-12-20 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 01-05-02.
	* Replace pageheadfoot option with pagehead.
	* Small updates to documentation.
2014-12-08 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 01-05-00.
	* First official release of the ATLAS preprint style.
	* atlasstyle is now default for all documents.
	* biblatex with the bibtex backend is the default way of typesetting references.
	* Use scrpage2 with KOMA-Script and fancyhdr with normal LaTeX classes.
	* Add template fles for TeX Live 2009 and central atlaslatex installations.
	* Remove date/time definition from atlasmisc.sty to avoid errors with TeX Live 2013.
	* Add a document on table formatting.
	* Clean up paper template and change its name to a general guide.
	* Bring biblatex and bibtex onto a similar level in the documentation and the style file.
	* Harmonise biblatex and BibTeX style files. Style conforms to ATLAS wishes.
	* Add option to use different backends with biblatex in atlaspackage.
	* Revise a bit the documentation on a BibTeX entry for a CONF note.
	* Add date to CERN preprint front page.
	* Move biblatex style file to latex subdirectory and just link from bibtex/bst.
	* Add options to turn on/off title and style of title for articles with biblatex.
	* Add heavy ion style file. A few new definitions aded to atlasmisc.sty.
	* Auxiliary material includes fancyhdr or scrpage2 by default.
	* Start adding standard text snippets.
	* Small fix to detector description.
2014-11-20 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 01-04-01.
	* Small fix so atlascover recognises better when atlasdoc is used.
	* Started documenting ATLAS preprint style in atlas_latex.
2014-11-19 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 01-04-00.
	* First implementation of the ATLAS preprint style.
	* Fonts still have to be checked on other platforms.
	* Major rewrite of both atlasdoc.cls and atlascover.sty, which removes spurious offsets.
	* Removed need for title skip parameter and horizontal and vertical offsets on cover pages.
	* Need coverpage=true in atlascover.sty if you want a draft cover and are using
	  atlascover.sty standalone.
	* No longer need atlasdoc as option to atlascover,
	  as package checks if atlasdoc is being used itself.
	* make cleanpdf command added (or being added) to standard Makefiles.
	* Adding of extra blank pages after cover page mostly removed.
	  Have to see if it is necessary somewhere.
	* Options added to atlasdoc for different fonts.
	* showframe option added for debugging.
2014-10-20 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 01-03-06.
	* Require hyperref in atlascover to avoid problems with supporting documentation.
2014-10-16 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 01-03-05.
	* Rename documentation directories and files to use _ instead of -.
2014-10-09 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 01-03-04.
	* Small fix to auxiliary material.
	* Replace some \\ with \par in atlascover for consistency.
2014-10-09 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 01-03-03.
	* Fix to CONF and PUB note draft cover pages.
2014-09-22 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 01-03-02.
	* Instructions for Fedora added.
	* Do not use lineno with revtex - use class option linenumbers instead.
	* Add option to atlaspackage to turn off lineno.
	* Use \linewidth instead of \textwidth in PrintAtlasContribute so it works in 
	  two column format.
	* Print out web page on auxiliary material cover.
	* Fix typo that put line numbers on cover page.
	* Move date and page number from header to footer in draft mode.
	* List of contributors was too wide.
	* Small fix to BibTeX style files and bring them back in sync.
2014-09-15 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 01-02-00
    * Bug fixed for CentOS/Fedora, as scrdate/scrtime did not work properly.
2014-09-09 Ian Brock <Ian.Brock@cern.ch>
	* Add texmf swtich to atlasdoc (needed for cover).
	* full option did not work in atlaspackage.
	* Use kvoptions in atlascontribute.
	* Change option from noauthblk to authblk=false.
	* Internally quite a lot of variable name changes.
	* Prepare atlasdoc for moving to kvoptions.
	* Switched from tabs to spaces in many places.
2014-09-08 Ian Brock <Ian.Brock@cern.ch>
	* Small fix to atlaspackage so texlive switch works.
2014-09-06 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 01-01-00
	* Add template for auxiliary material (atlas-auxmat).
	* Add switch so that TeX Live 2009 also works.
	* Do not include atlascontribute in metadata file.
	* Add preprintcover to Makefile.
	* Use fancyhdr to make header in draft mode (and also for auxiliary material).
	* Use scrdate and scrtime for current date and time.
	* Replace color with xcolor.
	* Switch to kvoptions in atlaspackage.
	* Add option to atlaspackage to turn off including siunitx.
	* Added atlasjournal and atlasxref to atlasphysics.
	* Further improvements to documentation, especially to atlas-latex.
2014-09-04 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 01-00-00
	* Add some examples of paper drafts with journal formatting.
	* More style files for journal names and cross references.
	* Use kvoptions for setting options, as then offsets can be given.
	* Move logos from figures to logos directory.
	* Include JHEP BibTeX style file in bibtex/bst.
	* Updates to documentation, especially BibTeX and LaTeX guide.
2014-08-29 Ian Brock <Ian.Brock@cern.ch>
	* Added a new style file atlascontribute.sty. It can be used to create both the
	  list of authors and the contributions they made to the analysis.
	* atlas-document-contribute is no longer needed. This information should be
	  included in atlas-document-metadata.tex instead.
2014-08-28 Ian Brock <Ian.Brock@cern.ch>
	* Add lineno as required package, so that atlasdoc does not need atlaspackage.
	* Rounding note added to documentation.
2014-08-27 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 00-97-00.
	* atlas-physics document list of definitions created automatically.
	* CONF and PUB are now options for CONF and PUB notes.
	* Cover pages change a bit depending on these options.
	* EdBoard replaced by Readers for a PUB note.
	* More documentation on options in atlasdoc and atlascover added to atlas-latex
2014-08-27 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 00-96-00.
	* Merge biblatex setup into atlaspackage with an option.
	* Add option texmf to atlasphysics if package in installed centrally
	* Add note number back into title page
	* Switch back from \AtlasTitle to \title
	* Further improve documentation
2014-08-22 Ian Brock <Ian.Brock@cern.ch>
	* Tag as version 00-95-00.
	* First alpha release of atlaslatex.
	* atlasphysics.sty split into smaller files.
	* Options to steer atlasphysics.sty.
	* Documentation reorganised. Split into paper style,
	  for which PubCom is responsible and atlaslatex guide.
	* Templates all in templates directory.
	* Makefile can make a new document.
	* Better use of geometry to set page size everywhere.
	* Add inputenc and fontenc to atlasphysics.sty.
	* In fact, these (and txfonts) should probably move to atlasdoc.cls.
	* Use tocloft for table of contents.
	* Titles should invoke boldmath automatically.
2014-08-25 Ian Brock <Ian.Brock@cern.ch>
	* Merge biblatex into atlaspackage and add biblatex option.
	* Add koma option to atlasdoc.cls.


==> Makefile <==
# Makefile for creating an ATLAS LaTeX document

# Copyright (C) 2002-2020 CERN for the benefit of the ATLAS collaboration
#------------------------------------------------------------------------------
# By default makes mydocument.pdf using target run_pdflatex.
# Replace mydocument with your main filename or add another target set.
# Adjust TEXLIVE if it is not correct, or pass it to "make new".
# Replace BIBTEX = biber with BIBTEX = bibtex if you use bibtex instead of biber.
# Adjust FIGSDIR for your figures directory tree.
# Adjust the %.pdf dependencies according to your directory structure.
# Use "make clean" to cleanup.
# Use "make cleanpdf" to delete $(BASENAME).pdf.
# "make cleanall" also deletes the PDF file $(BASENAME).pdf.
# Use "make cleanepstopdf" to remove PDF files created automatically from EPS files.
#   Note that FIGSDIR has to be set properly for this to work.

# Set the default target to run_latexmk instead of run_pdflatex to use latexmk to compile.

# You can use the target version to check your TeX Live version.

# If you have to run latex rather than pdflatex adjust the dependencies of %.dvi target
#   and use the command "make run_latex" to compile.
# Specify dvipdf or dvips as the run_latex dependency,
#   depending on which you want to use.

#-------------------------------------------------------------------------------
# Check which TeX Live installation you have with the command pdflatex --version
TEXLIVE  = 2016
LATEX    = latex
PDFLATEX = pdflatex
# BIBTEX   = bibtex
BIBTEX   = biber
DVIPS    = dvips
DVIPDF   = dvipdf
TLVERS   = $(shell pdflatex --version | grep -Go 'TeX Live [0-9]*' | grep -Go '[0-9].*')
# TLOKAY   = $(shell test $(TLVERS) -ge $(TEXLIVE) && echo true)
TWIKI    = https://twiki.cern.ch/twiki/bin/view/AtlasProtected/PubComLaTeXFAQ

#-------------------------------------------------------------------------------
# The main document filename
BASENAME = ANA-GENR-2018-01-PAPER

#-------------------------------------------------------------------------------
# Adjust this according to your top-level figures directory
# This directory tree is used by the "make cleanepstopdf" command
FIGSDIR  = figs
#-------------------------------------------------------------------------------

# EPSTOPDFFILES = `find . -name \*eps-converted-to.pdf`
rwildcard=$(foreach d,$(wildcard $1*),$(call rwildcard,$d/,$2) $(filter $(subst *,%,$2),$d))
EPSTOPDFFILES = $(call rwildcard, $(FIGSDIR), *eps-converted-to.pdf)

# Default target - make mydocument.pdf with pdflatex
# default: run_pdflatex
# Use latexmk instead to compile
default: run_latexmk

.PHONY: run_latexmk
.PHONY: newdocument newnotemetadata newpapermetadata newfiles
.PHONY: draftcover preprintcover newdata
.PHONY: version clean cleanpdf help

# Check TeX Live version
version:
	@echo "Checking version"
	@echo "TLVERS $(TLVERS), TEXLIVE $(TEXLIVE)"
	if [ $(TLVERS) -lt $(TEXLIVE) ]; then \
		echo "Your TeX Live version ($(TLVERS)) is older than $(TEXLIVE). Please consult $(TWIKI)"; \
	fi

# Standard pdflatex target
run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Remove -pdf option to run latex instead of pdflatex
run_latexmk:
	latexmk -pdf $(BASENAME)

#-------------------------------------------------------------------------------
# Specify the tex and bib file dependencies for running pdflatex
# If your bib files are not in the main directory adjust this target accordingly
#%.pdf:	%.tex *.tex bib/*.bib
%.pdf:	%.tex *.tex *.bib
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<
#-------------------------------------------------------------------------------

# Default is to make a new paper
new: newnote

newpaper: TEMPLATE=atlas-paper
newpaper: newdocument newfiles newpapermetadata newauxmat

# newpapertexmf: TEMPLATE=atlas-paper
# newpapertexmf: newdocumenttexmf newfiles newpapermetadata newauxmat

newnote: TEMPLATE=atlas-note
newnote: newdocument newfiles newnotemetadata

# newnotetexmf: TEMPLATE=atlas-note
# newnotetexmf: newdocumenttexmf newfiles newnotemetadata

newbook: TEMPLATE=atlas-book
newbook: newdocument newfiles newpapermetadata

# newbooktexmf: TEMPLATE=atlas-book
# newbooktexmf: newdocumenttexmf newfiles newpapermetadata

draftcover:
	if [ $(TEXLIVE) -ge 2013 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' template/atlas-draft-cover.tex \
	    >$(BASENAME)-draft-cover.tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  cp  template/$(BASENAME)-draft-cover.tex $(BASENAME)-draft-cover.tex; \
	fi

preprintcover:
	sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' template/atlas-preprint-cover.tex \
	  >$(BASENAME)-preprint-cover.tex
	#cp template/atlas-preprint-cover.tex $(BASENAME)-preprint-cover.tex

newdata:
	sed s/atlas-document/$(BASENAME)/ template/atlas-hepdata-main.tex | \
	sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME)-hepdata-main.tex
	cp template/atlas-hepdata.tex $(BASENAME)-hepdata.tex

newdocument:
	if [ $(TEXLIVE) -ge 2013 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex | \
	    sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME).tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex >$(BASENAME).tex; \
	fi

# newdocumenttexmf:
# 	if [ $(TEXLIVE) -ge 2013 -a $(TEXLIVE) -lt 2100 ]; then \
# 	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex | \
# 	  sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' | \
# 	  sed 's/\\newcommand\*{\\ATLASLATEXPATH}{latex\/}/% \\newcommand\*{\\ATLASLATEXPATH}{latex\/}/' | \
# 	  sed 's/% \\newcommand\*{\\ATLASLATEXPATH}{}/\\newcommand\*{\\ATLASLATEXPATH}{}/' \
# 	  >$(BASENAME).tex; \
# 	else \
# 	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
# 	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex >$(BASENAME).tex; \
# 	fi

newpapermetadata:
	cp template/atlas-paper-metadata.tex $(BASENAME)-metadata.tex

newnotemetadata:
	cp template/atlas-note-metadata.tex $(BASENAME)-metadata.tex

newfiles:
	echo "% Put you own bibliography entries in this file" > $(BASENAME).bib
	# touch $(BASENAME).bib
	touch $(BASENAME)-defs.sty

newauxmat:
	cp template/atlas-auxmat.tex $(BASENAME)-auxmat.tex
	cp template/atlas-hepdata.tex $(BASENAME)-hepdata.tex

run_latex: dvipdf

# Targets if you run latex instead of pdflatex
dvipdf:	$(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $<
	@echo "Made $(basename $<).pdf"

dvips:	$(BASENAME).dvi
	$(DVIPS) $<
	@echo "Made $(basename $<).ps"

# Specify dependencies for running latex
#%.dvi:	%.tex tex/*.tex bibtex/bib/*.bib
%.dvi:	%.tex *.tex *.bib
	$(LATEX)    $<
	-$(BIBTEX)  $(basename $<)
	$(LATEX)    $<
	$(LATEX)    $<

%.bbl:	%.tex *.bib
	$(LATEX) $<
	$(BIBTEX) $<

help:
	@echo "To create a new paper/CONF Note/PUB Note draft give the command:"
	@echo "make newpaper [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "To create a new ATLAS note draft give the command:"
	@echo "make newnote [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "To create a long document (book) like a TDR:"
	@echo "make newbook [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo ""
	@echo "To compile the paper give the command"
	@echo "make"
	@echo "If your bib files are not in the main directory, adjust the %.pdf target accordingly." 
	@echo ""
	@echo "To compile the document using latexmk give the command:"
	@echo "make latexmk"
	@echo "You can also adjust the 'default' target."
	@echo ""
	# @echo "If atlaslatex is installed centrally, e.g. in ~/texmf:"
	# @echo "make newpapertexmf|newnotetexmf|newbooktemf [BASENAME=mydocument] [TEXLIVE=YYYY]"
	# @echo ""
	@echo "If you need a standalone draft cover give the commands:"
	@echo "make draftcover [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-draft-cover"
	@echo ""
	@echo "If you need a standalone preprint cover give the commands:"
	@echo "make preprintcover [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-preprint-cover"
	@echo ""
	@echo "If you need a document for HepData material give the commands:"
	@echo "make newdata [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-hepdata-main"
	@echo ""
	@echo "make clean    to clean auxiliary files (not output PDF)"
	@echo "make cleanpdf to clean output PDF files"
	@echo "make cleanps  to clean output PS files"
	@echo "make cleanall to clean all files"
	@echo "make cleanepstopdf to clean PDF files automatically made from EPS"
	@echo "make version to check your TeX Live version"
	@echo ""

clean:
	-rm *.dvi *.toc *.aux *.log *.out \
		*.bbl *.blg *.brf *.bcf *-blx.bib *.run.xml \
		*.cb *.ind *.ilg *.inx \
		*.synctex.gz *~ *.fls *.fdb_latexmk .*.lb spellTmp 

cleanpdf:
	-rm $(BASENAME).pdf 
	-rm $(BASENAME)-draft-cover.pdf $(BASENAME)-preprint-cover.pdf
	-rm $(BASENAME)-hepdata-main.pdf

cleanps:
	-rm $(BASENAME).ps 
	-rm $(BASENAME)-draft-cover.ps $(BASENAME)-preprint-cover.ps
	-rm $(BASENAME)-hepdata-main.ps

cleanall: clean cleanpdf cleanps

# Clean the PDF files created automatically from EPS files
cleanepstopdf: $(EPSTOPDFFILES)
	@echo "Removing PDF files made automatically from EPS files"
	-rm $^


==> sections/5_PO-Gitlab_and_CI_tools.tex <==
% !TEX root = ../ANA-GENR-2018-01-PAPER.tex
% Turn off some chktex warnings.
% chktex-file 1 chktex-file 8 chktex-file 46

%------------------------------------------------------------------------------
\section{PO-GitLab and CI tools}%
\label{sec:PO-Gitlab_and_CI_tools}
%------------------------------------------------------------------------------

The ATLAS Physics Office GitLab tools (\pogitlab) simplify the publication process of ATLAS documents by using the features provided by the CERN GitLab platform.

Previously, the publication workflow involved a heavy email exchange between ATLAS editors and the Physics Office in order to ensure that ATLAS rules were being followed up to submission of the paper to the arXiv and any peer-review journal.
This approach led, usually, to modifications by different parties (officers and editors), which were sometimes incorrect or conflicting and which slowed the publication process down. Due to the uniform and repetitive nature of the tasks required to submit a publication, an automatic tool was favored.

Three main tasks are handled by the GitLab integration tools throughout the submission phase: the automatic creation of GitLab repositories; the continuous verification of technical rules by the GitLab Continuous Integration (CI) tools; and the automatic processing of the document itself for submission. These tasks are presented at detail in this section.

%------------------------------------------------------------------------------
\subsection{GitLab structure to organize analysis groups and repositories}%
\label{sec:Gitlab_structure_to_organise_Analysis_groups_and_repositories}

A hierarchy of groups were created in GitLab to reflect the current ATLAS group organization. Each Physics or Combined Performance group, System Detector Project, and Activity is labelled as a category with four letters in the FENCE systems.
For example, the Top Quark physics group is {TOPQ}, and the Electron/Photon Combined Performance group is {EGAM}.
At the beginning of Phase~0, Git repositories are created in GitLab in the area corresponding to the lead group of the analysis.
The identifier of a Phase~0 entry is labelled ANA-GROUP-YEAR-NN, where GROUP can be, for example {TOPQ} or {EGAM}, while {YEAR} is the year the document was created and {NN} is a two-digit counter. For instance, {ANA-SUSY-2019-04} represents the fourth analysis created in the SUSY group in 2019.

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.9\textwidth]{Fig7}
  \caption{The substructure of a {HIGG} GitLab repository subgroup.
  The main admin group, {atlas-physics-office}, is shown at the top.
  The {HIGG} subgroup is selected, and its {ANA-HIGG-2017-08} subgroup is expanded.
  A repository for the paper and one for the internal note ({INT1}) are created under {ANA-HIGG-2017-08}.}%
  \label{fig:Gitlab_repository}
\end{figure}

In GitLab, the following labels are adopted: 
\begin{itemize}
    \item 
{ANA-GROUP-YEAR-NN-INTn} for internal note repository,
\item
{ANA-GROUP-YEAR-NN-PAPER} for a paper repository.
\end{itemize}
The other publication categories (e.g. PUB and CONF) are also included.
For instance, in the Higgs ({HIGG}) physics group, for a given {Phase~0} analysis entry {ANA-HIGG-2017-08},
\pogitlab will host ANA-HIGG-2017-08-INT1,2,...,n and ANA-HIGG-2017-08-PAPER.
This is illustrated in \Cref{fig:Gitlab_repository} where the GitLab interface is shown.
{ANA-HIGG-2017-08}, an analysis within the {HIGG} group, contains for example one paper and one internal note repository, respectively {ANA-HIGG-2017-08-PAPER} and {ANA-HIGG-2017-08-INT1}.

The automatic creation of repositories is done via communication between the FENCE framework and the GitLab API, which is explained in more detail in \Cref{sec:FENCE-Gitlab_Integration}.
The structure of groups also permits the definition of an LDAP (Lightweight Directory Access Protocol) based fine-grained access control provided by GitLab. It guarantees that repositories created under a given group are restricted to the appropriate set of users (group conveners, analysis participants, and PO officers).

\subsection{Automatic document creation}%
\label{sec:Automatic_document_creation}

The initial files and directories present in a repository created through the FENCE web interfaces are based on a template. They have their variables substituted according to requirements of the related publication in the moment of creation.
This way, all created repositories contain the default documents, correctly formatted, to start writing a paper, CONF note, PUB note, or INT note.
The repository is also configured with a protected branch named {PO-ready}, to which only members with the {Maintainer} role are allowed to push and merge. This special branch is used to run the final submission pipeline when the document is ready and has been reviewed by the relevant parties. The {master} branch is used as the main work branch, unprotected at the time of the repository creation, allowing all editors to push new commits and interact with the repository.

%------------------------------------------------------------------------------
\subsection{Continuous checks with GitLab CI}%
\label{sec:Real-time_check_with GitLabs_CI}

GitLab CI tools are designed to automatically execute a set of tasks every time a new modification is introduced into the document, which happens on every new commit pushed to the document repository.
A command line tool called \pogitlab was developed to perform a variety of checks on a given document.
Those checks verify distinct aspects of an ATLAS publication, from style guidelines to internal conventions, and is implemented in Python.
The application architecture is based on the isolation of each component that performs the verifications in abstractions that represent a job from the pipeline. Each job is represented as a single code path which can be executed without affecting the others, which allows for new and more complex tasks to be added continuously, and facilitates the reuse of each component for creating new pipelines.
Finally, the tool is packaged up in a Docker~\cite{docker} image which makes possible to run it in any environment that has Docker installed in it, beyond only the GitLab CI machines installed at CERN.

GitLab's CI offers a way to configure and organize task pipelines. A pipeline is simply a set of jobs grouped into different stages. All the jobs in the same stage are executed in parallel, while each stage is only executed after the previous one has completed. It is possible to start the jobs of one stage only if the previous ones have finished successfully, or alternatively  only if one or more previous stages have failed. The tool starts a pipeline automatically based on the configuration put in place for a given repository -- normally this is done every time a new commit is pushed to the repository.

Different sets of checks are performed in each step of the publication process.
For editors, all work done before the paper submission (detailed in \Cref{sec:Paper_submission}) is monitored by the {editing-pipelines} shown in \Cref{fig:editing-pipeline}.
These pipelines are triggered by any push made from Git branches whose name does not start with {PO-}. The special branches using the {PO-} prefix are tracked by the {submission-pipelines} when a paper is considered ready for submission to the arXiv and the peer-review journal.

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.9\textwidth]{Fig8}
  \caption{The editing-pipelines. These four stages perform checks before a publication is ready for submission, with the first stage checking the version of the \pogitlab package itself, the second stage running checks related to \LaTeX~formatting, the third ensuring that the ATLAS rules are followed, and the last stage testing if the document builds correctly (without \LaTeX-related errors).}%
  \label{fig:editing-pipeline}
\end{figure}

%------------------------------------------------------------------------------
\subsection{Paper submission}%
\label{sec:Paper_submission}

The CI also produces the files required for paper submission, using dedicated pipelines similar to the editing ones.
These are called {submission-pipelines}. They are responsible for producing the final tarball, the set of files in an archived format (\texttt{tar.gz}) that will be sent to the journal or to a public repository for building public web pages.

A protected Git branch, named {PO-ready}, is created by default at the time of the setup of the paper repository.
When a paper is ready for submission, an editor creates a Merge Request
to the {PO-ready} branch. % ZLM I don't think it is *mandatory* that this MR comes from master, right?
When this request is accepted by a Physics Office officer, the paper submission pipelines are triggered.
In addition, any branch or tag created following the pattern {PO-*} triggers the paper submission pipelines.
These pipelines have, in addition to the previously described checks, a flattening of the LaTeX documents, grouping together all the necessary files for submission, as shown in \Cref{fig:submission-pipeline}. The flattening goes through the following steps:

\begin{enumerate}
\item all the source files are merged into a single \LaTeX\ source file;
\item all the comments in the \LaTeX\ source file are removed;
\item all the figures are renamed following the convention required by the journals;
\item any directory structure is removed.
\end{enumerate}

Tarballs suitable for submission to the arXiv and journals are created using \TeX~Live 2020 and 2017, respectively. The two different versions differ in their handling of the bibliography and references, and must be checked in order to avoid incompatibilities. The arXiv, at the time of this publication, requires \TeX~Live 2020, while some APS journals, for example, require \TeX~Live 2017.
Other tarballs contain files with plots and tables for posting on a public web page.
These tarballs are created as GitLab artifacts and can be downloaded by the corresponding editors and members of the Physics Office. In the submission tarballs, any auxiliary material (e.g. figures and tables not for submission) is not included.

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.9\textwidth]{Fig9}
  \caption{A {submission-pipeline}. From left to right, preparation stage jobs check the version of the CI tools, copy \File{bib} and \File{sty} files along with the flattened \LaTeX\ document to a special folder.
 Then all figures and tables are renamed and labelled according to the journal's specifications.
  At the final stage, the flattened document is updated with the newly named figures and tables.
  In the last two steps, the document is built, producing the \File{bbl} file needed for the journal and the tarballs for the public web pages.}%
  \label{fig:submission-pipeline}
\end{figure}




==> sections/6_Authorlists_Acknowledgements_and_ProofChecker.tex <==
% !TEX root = ../ANA-GENR-2018-01-PAPER.tex
% Turn off some chktex warnings.
% chktex-file 1 chktex-file 8 chktex-file 46

%------------------------------------------------------------------------------
\section{Author lists, acknowledgements, and the proof checker}%
\label{sec:Authorlists_Acknowledgements_and_ProofChecker}
%------------------------------------------------------------------------------
\subsection{Author lists and acknowledgements files}%
\label{sec:Author_lists_and_acknowledgments_files}


The author list, often written {authorlist} for convenience, is the inventory of qualified authors at a given date, which is called the reference date.
Every paper has an associated list of qualified authors with a reference date that corresponds to the creation date of that list during {Phase~1}, just before the first circulation of the draft document to the collaboration.
%Qualified authors are active physicists contributing to the maintenance and operation of the experiment. 
Between {Phase~1} and {Phase~2}, this author list may be updated or amended.
%some people may receive exceptional authorship because of their involvement in the analysis or the paper,
%even if they are not yet qualified as authors through the usual process.
%Therefore the author list is updated to include "exceptional" authors.
%The special cases are evaluated by the Authorship Committee (AC) and proposed for approval to the Spokesperson, who will agree or not with each exception after reviewing the proposal from the AC.
% ZLM I find a discussion of our authorship policy out of scope for this paper -- and some of the details aren't quite right here (e.g. qualified authors are not only active physicists)
This information is stored in the ATLAS database and managed by {FENCE}.
\Cref{fig:authorlist_generation} shows a portion of the full list of members, their affiliations, and the related metadata which are needed to generate the full report.

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.9\textwidth]{Fig10}
  \caption{The {FENCE} author list generation interface. From left to right, the list of institutions used as affiliations; in the center of the screen,  the authors (blurred) are listed; at the top of the page, the interface allows the users to view (orange boxes) the creation date (left) for a given paper, the title of the paper (center), and the formats available for download (\File{tex}, \File{xml}, \File{pdf}, etc.; top right). As an example, two authors of this paper are highlighted with their affiliations (black boxes).}%
  \label{fig:authorlist_generation}
\end{figure}

% ZLM "agreed to include" can be read as having a negative connotation -- we don't want to voluntarily, but we've agreed to do so
The acknowledgements are incorporated in a short section that the collaboration includes in each paper to thank funding agencies for their financial support.
They do not change often, but they may add or remove a funding agency or a foundation at a given date.
Therefore, similarly to the author list, the acknowledgement file is built for each paper at a reference date.

Both files, the author list and the acknowledgements, are built using the {FENCE} framework and are automatically pushed to the appropriate GitLab repository, using the FENCE--\gitlab integration (\Cref{sec:FENCE-Gitlab_Integration}).
Their integration into the paper is straightforward at the time of submission to a journal.
FENCE provides the MBF infrastructure to retrieve the required information from the database (see \Cref{sec:FENCE_main_concepts}) and build all the files.

The author list is built by the {FENCE} framework into an xml file. This is composed of three main blocks:
\begin{itemize}
\item Header: stores the paper's main information.
\item Institutes: the list of institutes and their InSPIRE-HEP references.
\item Authors: the list of authors and their identifying information, including names, initials, affiliations, and ORCID\footnote{ORCID stands for Open Researcher and Contributor ID.}.
\end{itemize}

Most journals accept the \File{xml} version of the author list as input, and retrieve all the needed data from it.
The complete set of author lists created for every ATLAS paper that has been submitted or published since 2009 is accessible through a web interface, called the {FENCE} author list interface.
They are easily filtered using a search box.

The acknowledgement \File{tex} file is built using a standard template and is filled using the {FENCE} framework to retrieve the required information about the ATLAS funding agencies.

%------------------------------------------------------------------------------
\subsection{Proof checker functionalities}
\label{sec:Proof_checker_functionalities}

Once the author list included in the tarball has been sent to the journal, a check is made to determine whether the publisher has correctly used the provided information.
This check involves a comparison of the proof \File{pdf} file that was sent back to the ATLAS Collaboration for review to the original \File{xml/tex} file.
This process used to be done by hand, requiring the PO officer to check that each of the approximately 3000 authors and 200 institutes were correctly reported and matched.
The proof checker is the tool provided for ATLAS to compare these two files automatically.
A report of this comparison, one for every version of the proof, is available to PO officers who check the results. 

The proof checker follows this process:

\begin{itemize}
\item retrieve the information from the \File{xml} file, containing the authors and their affiliations;
\item extract the text from the journal's \File{pdf} file;
\item parse the text from the \File{pdf} file, creating the target reference;
\item compare the official reference obtained from the \File{xml} file with the target reference;
\item create a report with the differences found between the original and the target reference;
\item link the report to the main ATLAS report page.
\end{itemize}

The main difficulty with this process involves extracting the content from the \File{pdf} file; the text is not easily retrieved, for a variety of reasons.
One is that many elements have to be identified and ignored, such as row numbers, watermarks, footers, and headings.
Another reason is that words extracted from a \File{pdf} file don't follow a specific coding convention;
the file can contain non-ASCII characters that can be extracted in many different ways.
The \File{pdf} file can specify a predefined encoding standard to use, or provide a lookup table of differences between predefined and alternative encoding standards;
for texts with uncommon Latin characters, which are routine in this kind of publication,
special encoding is used, and they are translated into the Unicode standard convention for glyph representation. It is necessary to provide a ToUnicode Table, to map the codes used in the \File{pdf} file to Unicode symbols, where semantic information about the characters is preserved.
The proof checker also has to parse all the publication text and recognize where the author list starts, where it ends, where the institute list starts and where it ends.
All this is made more difficult by the fact that different publishers have different layouts and create different versions of \File{pdf} files.
This makes the above problems not generic,
but often specific to a particular publisher.

After the target reference is created, the comparison looks for:
\begin{itemize}
\item authors that seem to be missing from the \File{pdf} file.
  Here, false positives are often due to character encoding and spaces;
\item authors with inconsistent punctuation.
  This section points out differences between original and target references authors' first name punctuation,
  which can follow the rules {X}. or {X.Y.} or {X.-Y.} or {X-Y.} with or without spaces;
\item institutes that seem to be missing from the \File{pdf} file.
  Here false positives are often due to the difficulties extracting and correctly encoding/decoding special glyphs in the \File{pdf} file format, which make the comparison fail;
\item institutes with close matches. All the entries that look like the original but have some inconsistencies land in this group.
  Some publishers replace, for example, ``USA'' with ``United States of America'' (or vice versa).
  Sometimes there is a new character that doesn't corrupt the institute entry,
  but makes the match imperfect, for example, ``Università'' and ``Universit`a''; this is one of the problems that often occurs due to the difficulties of extracting data automatically from a pdf file. 
\item mismatched authors. All the authors collaborate through one or more institutes.
  The link between the author and the institute is checked for consistency.
  This sometimes results in a false positive,
  because it is not always easy to extract from the \File{pdf} file the index number of an institute,
  mainly because the text coming from the journal \File{pdf} file also includes other elements such as line numbers of the document.
  For this reason an author originally assigned to institute number {X} can end up matched with target institute {YX},
  because in the text extracted from the {pdf} the number {X} might be preceded by a {Y} line number;
  institute {YX} may not exist;
\item deceased authors. In some cases, ATLAS has tagged authors as deceased but the publication fails to mark them as such, or vice versa;
\item missing funding agencies, or those wrongly added by the publisher.
\end{itemize}

In early 2019, due to changes in CERN systems, the component written in Prolog which ran the comparison went out of service.
This implied an urgent need for a new tool for this task. Python was chosen as the programming language for the new comparison engine.

A way to obtain the best match among all the items of an array of institutes and authors was sought,
because one cannot rely on finding an author or institute in the same position of the sequences in the \File{xml} and \File{pdf} files.
For this purpose the concept of Levenshtein distance~\cite{Levenshtein_SPD66} was applied,
so that a weighted index of similarity can be obtained to decide what is matched with what, and to then effectively check for anomalies.
The Levenshtein distance between two words is the minimum number of single-character edits, such as insertions, substitutions or deletions, required to change one word into the other.
For example the Levenshtein distance between ATLAS and Atlassian is 4 (4 insertions); between Maurizio and Fabrizio is 2 (2 substitutions); raise and race is 2 (1 deletion, 1 substitution).

Mathematically, the Levenshtein distance lev$_a$$_,$$_b$(|a|,|b|) between two strings a and b of length |a| and |b| respectively is given by:

$$ \mathrm{lev}_{a,b}(i,j)=
\begin{cases}
 \max(i,j) & \text{ if } \min(i,j)=0, \\
 \min \begin{cases}
    \mathrm{lev}_{a,b}(i-1,j) +1 \\
    \mathrm{lev}_{a,b}(i,j-1) +1 \\
    \mathrm{lev}_{a,b}(i-1,j-1) +1_{(a_i\not = b_j)} 
    \end{cases}& \text{ otherwise,}
\end{cases}$$

\noindent where 1$_{(a_i \neq b_j)}$ is equal to 0 when a$_i$ = b$_j$ and equal to 1 otherwise, and lev$_a$$_,$$_b$(i,j) is the distance between the first i characters of a and the first j characters of b.

A feature was developed to help the script evaluate as correct matches some that would not otherwise appear to be such.
A list of synonyms (see \Cref{sec:Proof_checker_synonyms}) is created for every entry, author or institute,
to teach the proof checker to validate similar strings when the differences are due only to problems from decoding the text from the \File{pdf} file.
So, for instance, if author X.~Nonamečič is not found in the target reference,
but from the \File{pdf} entries an author with name X.~Nonamež ciž c appears, then,
as it has been previously verified that in the \File{pdf} file the name appears as expected, the proof checker considers it to be the same, and skips the problem.
A very long list of false positives can be found in the report page as \enquote{skipped items}.
The list of synonyms is updated manually, but a tool, the Synonym web page, has been created to allow users to update this list themselves.

%------------------------------------------------------------------------------
\subsubsection{Proof checker synonyms}%
\label{sec:Proof_checker_synonyms}

As previously discussed, the comparison between the \File{pdf} file and the \File{xml} file can generate false positives.
To minimize the list of false positives in the report page, the proof checker includes a synonyms list that allows the comparison script to understand if the difference is a real error or another correct way to display the same information. An example of a working synonym is
{\small Physics Department, SUNY Albany, Albany {\bf NY, United States of America}} for the ATLAS original version and 
{\small Physics Department, SUNY Albany, Albany, {\bf New York, USA}} for the Journal version. These differences are acceptable, since the main information is correctly displayed. All the synonym records are managed using a JSON file and are separated into institutes and authors.
Institute listings are, for example:
\begin{lstlisting}
{
    "id": "2", 
    "original": "Department of Physics, University of Alberta, Edmonton AB, Canada"
    "synonyms": ["Department of Physics, University of Alberta, Edmonton, Alberta, Canada"],
}
\end{lstlisting}
\noindent Author listings are, for example:
\begin{lstlisting}
{
    "original": "A. B\\\"ub",
    "inspire": "INSPIRE-00000000", 
    "foafName": "A Bub"
    "synonyms": ["A. B\u00f2b", "A. B\u00a8 b"], 
}
\end{lstlisting}

\begin{figure}[htb]
  \centering
  \includegraphics[scale=0.65]{Fig13}
  \caption{Proof checker synonyms. One can search for an item and see all the defined synonyms for institutes and authors' names.}
  \label{fig:synonym_webpage}
\end{figure}

To manage the list of proof checker synonyms, ATLAS provides a web interface that allows users to search for an existing entry and manage the recorded synonyms.
Searching for an institute or author will display the list of records that match the search criteria (see \Cref{fig:synonym_webpage}).  This allows PO officers to edit the synonyms for the record.
Clicking the edit icon shows a new page section where a new synonym can be added.
After confirmation, this is added to the list of synonyms and is taken into account by the next run of the proof checker.

%------------------------------------------------------------------------------
\subsubsection{Report page}
\label{sec:Report_page}

The proof checker provides a report for each paper and draft version (the journal may produce several proofs).
This report is provided and stored in a JSON file and must be parsed to show the report results in a human-readable way.
The report contains all the paper information and the comparison results sorted by topic, for example:
\begin{lstlisting}
{
    "ref_code": "EXOT-2017-24",
    "ref_date": "2018-07-31", 
    "creation_date": "29-Oct-2018",
    "publisher": "'APS'", 
    "document": "doc1053",
    "filename": "LY15578_proof_v2", 
    "authors_missing_skip": [...], 
    "authors_missing_list": [...],
    "authors_puntuation_list": [...]
    "institutes_missing_pdf_list": [...], 
    "institutes_missing_pdf_skip": [...], 
    "authors_mismatched_list": [...], 
    "authors_not_deceased_list": [...], 
    "authors_deceased_list": [...], 
    "institutes_close_matches_list": [...], 
    "founding_agencies_missing": [...],
    "founding_agencies_wrong": [...]
}
\end{lstlisting}
The JSON file contains more information than is displayed; the information is reduced to allow the web page to optimize the display of the huge amount of information and to retain data for future improvements.
The web page contains some hidden sections that are produced by the proof checker via the known synonyms.
These can be displayed by clicking on \enquote{Skipped +}.
Here the page will show all the false positive results that the proof checker found in its comparison, but that are ignored after association with the synonyms.

The proof checker helps the Physics Office staff in a tedious task, but it is far from being a perfect tool. It requires continuous maintenance and updates for new cases,
changes in publication layouts, and new conventions in the author lists and their format.
Further improvements are planned, with the goal of minimizing the number of cases to be checked manually.


==> sections/7_Handling_the_metadata.tex <==
% !TEX root = ../ANA-GENR-2018-01-PAPER.tex
% Turn off some chktex warnings.
% chktex-file 1 chktex-file 8 chktex-file 46

%------------------------------------------------------------------------------
\section{Handling the metadata}
\label{sec:Handling_the_metadata}
%------------------------------------------------------------------------------

%----------------------------------------------------------------------

The ATLAS database stores data of various kinds that are displayed in different ways via web pages.
The {FENCE} framework provides an \textbf{\gls{API}} to retrieve this information.
A call to the \textbf{\gls{API}}, allowed after a user authentication, provides the results in a \textbf{\gls{JSON}} format.
This kind of information is easily parsed by most common programming languages and is standard for \textbf{\gls{API}} results.

There are 2 main ways to provide web pages:
\begin{itemize}
\item standard HTML pages;
\item include files for \textbf{\gls{TWiki}} pages.
\end{itemize}

They run on an ATLAS~PO \textbf{\gls{Virtual Machine}}, which provides scripts, \textbf{\gls{cron-jobs}}, or {HTML} pages to the users.
This \textbf{\gls{Virtual Machine}} is directly connected to the {FENCE} framework to use its \textbf{\gls{API}} and retrieve data, parse it, and store it in the \textbf{\gls{EOS}} ATLAS file system.


%------------------------------------------------------------------------------
\subsection{ATLAS data in public pages}
\label{sec:ATLAS_data_in_public_pages}

{FENCE} also allows members who do not belong to the ATLAS collaboration to access some of the information stored in its database.
It provides various ways to retrieve and show the information, through
a \textbf{\gls{cron-jobs}} that runs on the ATLAS~PO \textbf{\gls{Virtual Machine}} and extracts the data, parses it, and shows it to public.

An example in which the data are retrieved using the {FENCE} \textbf{\gls{API}} with a \textbf{\gls{cron-jobs}} on the ATLAS~PO \textbf{\gls{Virtual Machine}} is the ATLAS map web page, \Cref{fig:atlas_map_webpage}, where people can see a map of all active member institutes of the ATLAS collaboration.

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.9\textwidth]{Fig15}
  \caption{The ATLAS map web page. The numbers displayed at a regional level represent the count of  institutions.}
  \label{fig:atlas_map_webpage}
\end{figure}

This dynamic web page filters the results to use only the active institutes. This process is done using a \textbf{\gls{Python}} script, which makes a request to the \textbf{\gls{API}}, parses the results, and builds its own \textbf{\gls{JSON}} file. This file contains all the institute information (name, country, links, coordinates, etc.) and the layers to build the map. Once the \textbf{\gls{Python}} script builds the \textbf{\gls{JSON}} file, the output is interpreted by the web page, which takes care of displaying the layers and the markers for the institutes.


%------------------------------------------------------------------------------
\subsection{Data on {TWiki} pages}
\label{sec:Data_on_twiki_pages}

Displaying information on a \textbf{\gls{TWiki}} page requires the use of the \textbf{\gls{TWiki}} \texttt{\%INCLUDE<path>} function.
This function permits inclusion of the content of the \File{<path>} file that is interpreted by the \textbf{\gls{TWiki}} page.
The content can be \textbf{\gls{TWiki}} code or {HTML} code.
{HTML} code allows a more dynamic page to be created.
One can use \textbf{\gls{javascript}}, \textbf{\gls{jQuery}}, and other web development tools to make the content more intuitive to the user.
In this case the page will be loaded on-demand and the data will be displayed in real time via the {FENCE} framework.

\begin{figure}[htb]
  \centering
  \includegraphics[width=\textwidth]{Fig16}
  \caption{Public results \textbf{\gls{TWiki}} page. This page will show the lists of all types of ATLAS documents and allow users to filter the results using the section at the top of the page.}
  \label{fig:public_twikipage}
\end{figure}

The public results page, \Cref{fig:public_twikipage}, is an example of an {include} using an {HTML} page which retrieves data using the {FENCE} \textbf{\gls{API}} and displays it to the user into a \textbf{\gls{TWiki}} page.
This page shows the full list of documents stored in the ATLAS database and managed by the {FENCE} framework.
It also allows users to filter results using the buttons on the top of the page.
This page loads more then 1300 records with all the related information.
Retrieving all these records at once requires a lot of time.
To avoid this, the page initially loads only the first 10 records of each section and makes the page available for user interaction,
then in the background it loads the other records.
This solution allows the loading process to run faster and avoids users' having to wait for the complete data loading.


==> sections/8_Conclusion.tex <==
% !TEX root = ../ANA-GENR-2018-01-PAPER.tex
% Turn off some chktex warnings.
% chktex-file 1 chktex-file 8 chktex-file 46

%------------------------------------------------------------------------------
\section{Conclusion}
\label{sec:Conclusion}
%------------------------------------------------------------------------------

A suite of tools have been developed to support
the publication of documents by the ATLAS collaboration.
While the emphasis is on papers published in refereed journals,
the new technology also supports internal documents and other public documents such as conference and public notes.

The {FENCE} framework is used as the backbone of the whole setup
and is also used to interface the web-based tracking of the status of
an analysis with the documentation in GitLab.
Extensive use is made of the Continuous Integration tools available in GitLab to ensure that documents can easily be submitted to the arXiv and journals as soon as they have been approved by the collaboration.

The software solutions described in this document are now used to accompany the entirety of a physics analysis, from the expressions of interest by research groups to the final journal publication.
They also include the generation of the appropriate author list 
and processing of proofs.
In addition, metadata are continuously maintained, and public web pages and all the related information regarding the scientific results of the experiment are obtained automatically.

The tools are used by the whole collaboration and
minimize the amount of manual work required for repetitive procedures,
easing the workload of editors, editorial boards, management, and the Physics Office. At the same time, all documents connected to an analysis can now be accessed from a central tool where the experiment's rules and knowledge are codified and made available in an intuitive way. 

The FENCE framework and its integration with the most up to date and efficient tools has consequently provided a more professional and efficient automatized work environment to the entire collaboration.

